Multicast Communications in Tree Networks with Heterogeneous Capacity Constraints

A widely studied problem in communication networks is that of finding the maximum number of communication requests that can be scheduled concurrently, subject to node and/or link capacity constraints. In this paper, we consider the problem of finding the largest number of multicast communication requests that can be serviced simultaneously by a network of tree topology, subject to heterogeneous capacity constraints. This problem generalizes the following two problems studied in the literature: a) the problem of finding a largest induced $k$-colorable subgraph of a chordal graph, b) the maximum multi-commodity flow problem in tree networks. The problem is already known to be NP-hard and to admit a $c$-approximation ($c \approx 1.58$) in the case of homogeneous capacity constraints. We first show that the problem is much harder to approximate in the heterogeneous case. We then use a generalization of a classical algorithm to obtain an $M$-approximation where $M$ is the maximum number of leaves of the subtrees representing the multicast communications. Surprisingly, the same algorithm, though in various disguises, is used in the literature at least four times to solve related problems (though the analysis is different). The special case of the problem where instances are restricted to unicast communications in a star topology network is known to be polynomial-time solvable. We extend this result and show that the problem can be solved in polynomial time for a set of paths in a tree that share a common vertex.

==> MaxkColorableSet.tex <==
In this section, we consider the {\mkc} problem.

Given a chordal graph $G$, one can find a representation $\rep$ of it in polynomial time.
Let $\vect{k}$ be the vector with $k_e=n$ for every edge $e$ of $T$ and $k_v=k$ for every vertex $v$ of $T$.
We recall that, in this context, the following statements are equivalent:
\begin{itemize}
\item A subset $U$ of vertices of $G$ is $k$-colorable.
\item The set $\TT_U$ satisfies $\load(\TT_U,v) \leq k$ for every vertex $v$ of $T$.
\item The set $\TT_U$ is feasible for the instance $\inst$ of $\mstbl$.
\end{itemize}

Therefore, one can run $\alg$ on the instance $\inst$ to get an $M$-approximation for {\mkc} in chordal graphs where $M$ is the maximum number of leaves over all subtrees of a representation. 
Whenever $G$ is a $\vpt$ graph, one can find in polynomial time a representation $\TT$ in which every subtree is a path. 
Since the number of leaves of a path is at most $2$, we obtain the following corollary.

\begin{corollary}\label{coro:VptTwoApprox}
There is a 2-approximation algorithm for {\mkc} in {\vpt} graphs.
\end{corollary}


Since in a directed tree one of the two leaves of a path $T_i$ is $root(T_i)$, we obtain
\begin{corollary}\label{coro:DirectedPathOptimal}
{\mkc} can be solved optimally in directed path graphs.
\end{corollary}

We now proceed with two graph classes that are not chordal, namely {\ept} graphs and circular arc graphs. 
Since the chromatic number problem is $\nph$ for $\ept$ graphs \cite{GJ85} and also for circular arc graphs \cite{GJMP90-CircularArcGraphColoring},
by Corollary \ref{obs:ChromaticNPH}, the {\mkc} problem is $\nph$ when restricted to each of these graph classes.
We provide two constant approximation algorithms for these classes in Theorem \ref{thm:eptApprox} and Theorem \ref{thm:cagApprox}.

Since the recognition problem of $\ept$ graphs is $\nph$, in this section we assume that an {\ept} graph is given with a representation $\rep$.
\begin{theorem}\label{thm:eptApprox}
There is a $\frac{2k}{\left \lfloor \frac{2k}{3} \right \rfloor}$-approximation algorithm for {\mkc} in $\ept$ graphs.
\end{theorem}
\begin{proof}
Let $\opt$ be an optimal solution for {\mkc}, and let $\opt_1, \ldots, \opt_k$ be the color classes of some $k$-coloring of $\opt$.
Assume without loss of generality $\abs{\opt_1} \geq \abs{\opt_2} \geq \ldots \geq \abs{\opt_k}$.
Let $\opt' = \cup_{i=1}^{\lfloor 2k/3 \rfloor} \opt_i$.
Clearly,
\[
\abs{\opt'} \geq \frac{\lfloor 2k/3 \rfloor}{k} \abs{\opt}
\]
and $\opt'$ is $2k/3$-colorable. In particular, $\load(\opt',v) \leq 2k/3$ for every $v \in T$.
Let $\vect{k}$ be such that $k_e=2k/3$ for every edge $e$ of $T$, and $k_v=n$ for every vertex $v$ of it.
By running $\alg$ on the instance $(T,\TT,\vect{k})$, one gets a solution $\sol$ with maximum load at most $2k/3$.
In \cite{RaghavanUpfal94}, it is shown that every set of paths with maximum edge load at most $L_E$ can be colored using at most $3L_E/2$ colors.
Therefore, $\sol$ is $k$-colorable.
Furthermore, $\sol$ is a $2$-approximation for $\mstbl$.
We conclude, 
\[
\abs{\sol} \geq \frac{\abs{\opt'}}{2} \geq \frac{\lfloor 2k/3 \rfloor}{2k} \abs{\opt}.
\]
\end{proof}

\begin{theorem}\label{thm:cagApprox}
There is a $2$-approximation algorithm for {\mkc} in circular arc graphs.
\end{theorem}
\begin{proof}
Let $G=(V,E)$ be a circular arc graph represented as circular arcs of a circle $C$. 
Choose an arc $e$ of $C$ that is contained in a smallest set of circular arcs, and let $K_e$ be the clique of $G$ that corresponds to the circular arcs containing $e$.
Then $G[V \setminus K_e]$ is an interval graph.
Compute a maximum $k$-colorable set $S_I$ of $G[V \setminus K_e]$.
Let $S_e$ be a subset of $K_e$ with $\min (\abs{K_e},k)$ vertices.
We claim that a biggest set among $S_I$ and $S_e$ is a $2$-approximation.
Indeed, any $k$-colorable set $S \subset V$ is partitioned into two sets $S \cap K_e$ and $S \setminus K_e$, each of which is clearly $k$-colorable.
We conclude, 
\[
\abs{S}=\abs{S \setminus K_e}+\abs{S \cap K_e} \leq
\abs{S_I} + \abs{S_e} \leq 2 \max (\abs{S_I}, \abs{S_e}).
\]
\end{proof}
